Diffeomorphic Mesh Deformation via Efficient Optimal Transport for Cortical Surface Reconstruction

Mesh deformation plays a pivotal role in many 3D vision tasks including dynamic simulations, rendering, and reconstruction. However, defining an efficient discrepancy between predicted and target meshes remains an open problem. A prevalent approach in current deep learning is the set-based approach which measures the discrepancy between two surfaces by comparing two randomly sampled point-clouds from the two meshes with Chamfer pseudo-distance. Nevertheless, the set-based approach still has limitations such as lacking a theoretical guarantee for choosing the number of points in sampled point-clouds, and the pseudo-metricity and the quadratic complexity of the Chamfer divergence. To address these issues, we propose a novel metric for learning mesh deformation. The metric is defined by sliced Wasserstein distance on meshes represented as probability measures that generalize the set-based approach. By leveraging probability measure space, we gain flexibility in encoding meshes using diverse forms of probability measures, such as continuous, empirical, and discrete measures via varifold representation. After having encoded probability measures, we can compare meshes by using the sliced Wasserstein distance which is an effective optimal transport distance with linear computational complexity and can provide a fast statistical rate for approximating the surface of meshes. To the end, we employ a neural ordinary differential equation (ODE) to deform the input surface into the target shape by modeling the trajectories of the points on the surface. Our experiments on cortical surface reconstruction demonstrate that our approach surpasses other competing methods in multiple datasets and metrics.

==> tables/abs_trt_combine.tex <==
\begin{table}[t]
\parbox{.45\linewidth}{
\centering
\caption{
\textbf{White matter surface reconstruction consistency comparison} in terms of EMD, SWD, ASSD on TRT dataset.
}
% \scalebox{0.6}{
\resizebox{0.45\columnwidth}{!}{
\begin{tabular}{lccc}
    \toprule
        Method & EMD & SWD & ASSD  \\
    \midrule
        Vox2Cortex & .886 $\pm .130$  & .485 $\pm .176$  & .263 $\pm .112$ \\
        CortexODE & .799 $\pm .038$  & .444 $\pm .201$    & .241 $\pm .040$\\
        FreeSurfer  & .859 $\pm .213$ & \textbf{.358} $\pm .275$    & .286 $\pm .156$\\
    \midrule
        DD-SWD  & \textbf{.796} $\pm .041$   & .437 $\pm .194$   & \textbf{.237} $\pm .040$  \\
    \bottomrule
\vspace{-0.8em}
\end{tabular}
}
% \caption{Foo}
\label{tab:trt}
}
\hfill
\parbox{.5\linewidth}{
\centering
\caption{
\textbf{Ablation Study} in terms of EMD and SWD metric. \textit{P.S.} and \textit{O.V.} are short for \textit{point sampling} and \textit{oriented varifold} representation, respectively. Best values are highlighted. 
}
% \scalebox{0.6}{
\resizebox{0.5\columnwidth}{!}{
\begin{tabular}{lcccc}
\toprule
 & \multicolumn{2}{c}{Left WM} & \multicolumn{2}{c}{Right WM} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
     & EMD          & SWD      & EMD      & SWD      \\ 
\midrule
    SWD on P.S.       & 1.135 $\pm .112$ & .445 $\pm .212$ & 1.146 $\pm .046$ & .423 $\pm .218$ \\
    CD on O.V.     & .874 $\pm .121$ & .499 $\pm .343$ & .848 $\pm .077$ & .529 $\pm .209$  \\
    Sinkhorn on O.V.     & 1.023 $\pm .109$ & .578 $\pm .307$ & 1.002 $\pm .071$ & .568 $\pm .178$  \\
    \midrule
    SWD on O.V.       & \textbf{.802} $\pm .127$ & \textbf{.423} $\pm .379$ & \textbf{.791} $\pm .076$ & \textbf{.370} $\pm .232$ \\
\bottomrule
\vspace{-0.8em}
\end{tabular}
}
% \caption{Bar}
\label{tab:ablation}
}
\end{table}
